An empirical study on speech restoration guided by self supervised speech representation

Enhancing speech quality is an indispensable yet difficult task as it is often complicated by a range of degradation factors. In addition to additive noise, reverberation, clipping, and speech attenuation can all adversely affect speech quality. Speech restoration aims to recover speech components from these distortions. This paper focuses on exploring the impact of self-supervised speech representation learning on the speech restoration task. Specifically, we employ speech representation in various speech restoration networks and evaluate their performance under complicated distortion scenarios. Our experiments demonstrate that the contextual information provided by the self-supervised speech representation can enhance speech restoration performance in various distortion scenarios, while also increasing robustness against the duration of speech attenuation and mismatched test conditions.

==> backups.tex <==




\begin{equation}
        L_{total} = \frac{1}{T}{\left\| {s - \hat s} \right\|_1} + \lambda \sum\nolimits_{i = 1}^M {L_{stft}^{\left( i \right)}\left( {s,\hat s} \right)} 
    \label{eq:loss_all}
\end{equation}
where $L_{stft}$ is defined as
\begin{equation}
    \begin{array}{c}
    {L_{stft}} = {L_{sc}}\left( {s,\hat s} \right) + {L_{mag}}\left( {s,\hat s} \right),\\
    {L_{sc}}\left( {s,\hat s} \right) = \frac{{{{\left\| {\left| {STFT\left( s \right)} \right| - \left| {STFT\left( {\hat s} \right)} \right|} \right\|}_F}}}{{{{\left\| {\left| {STFT\left( s \right)} \right|} \right\|}_F}}},\\
    {L_{mag}}\left( {s,\hat s} \right) = \frac{1}{T}\left\| {\log \left| {STFT\left( s \right)} \right| - \log \left| {STFT\left( {\hat s} \right)} \right|} \right\|
    \end{array}
    \label{eq:loss_stft}
\end{equation}




\begin{table}[]
%\fontsize{9pt}{12pt}
%\selectfont
\begin{tabular}{|c|l|}
\hline
\textbf{Degradation}                                               & \multicolumn{1}{c|}{\textbf{Description}}                                                                             \\ \hline
Noise                                                              & \begin{tabular}[c]{@{}l@{}} noise segments are added at various SNRs \end{tabular} \\ \hline
Clipping                                                           & \begin{tabular}[c]{@{}l@{}} speech magnitudes are clipped with a \\random threshold ranging 0.06-0.9.\end{tabular}                                           \\ \hline
\begin{tabular}[c]{@{}c@{}}Limited   \\ bandwidth\end{tabular}     & \begin{tabular}[c]{@{}l@{}} bandwidths are limited with low-pass \\cutoff frequency ranging 4-8 kHz using \\Butterworth filters having orders of 2-10.\end{tabular}               \\ \hline
\begin{tabular}[c]{@{}c@{}}Time domain \\ discontinuity\end{tabular} & \begin{tabular}[c]{@{}l@{}}Random gains in 0-0.01 are applied to 1-20 \\durations ranging 10-50 ms.\end{tabular}                                                \\ \hline
\end{tabular}
\caption{List of degradation factors considered in this paper.}
\label{degradation}
\end{table}







\begin{table*}[t]
% \fontsize{9pt}{12pt}
% \selectfont
\begin{tabular}{|c|c|cc|cccc|cccc|}
\hline
\multirow{2}{*}{Type} & \multirow{2}{*}{Model} & \multicolumn{2}{c|}{Strategy} & \multicolumn{4}{c|}{VCTK-Denoising}                                                                                           & \multicolumn{4}{c|}{+   degradation factors}                                                                                  \\ \cline{3-12} 
                            &                               & Aug. & SSL & \multicolumn{1}{c|}{PESQ}          & \multicolumn{1}{c|}{NISQA}         & \multicolumn{1}{c|}{STOI}           & SISNR         & \multicolumn{1}{c|}{PESQ}          & \multicolumn{1}{c|}{NISQA}         & \multicolumn{1}{c|}{STOI}           & SISNR         
                            \\ \hline
\multirow{3}{*}{Masking}    & \multirow{3}{*}{BLSTM}        &       & & \multicolumn{1}{c|}{2.75}          & \multicolumn{1}{c|}{4.17}          & \multicolumn{1}{c|}{0.943}          & 17.9          & \multicolumn{1}{c|}{1.64}          & \multicolumn{1}{c|}{2.18}          & \multicolumn{1}{c|}{0.869}          & 9.8
\\ \cline{5-12} 
                            &                               & \checkmark &                   & \multicolumn{1}{c|}{2.79}          & \multicolumn{1}{c|}{4.18}          & \multicolumn{1}{c|}{0.944}          & 18.1          & \multicolumn{1}{c|}{1.86}          & \multicolumn{1}{c|}{2.42}          & \multicolumn{1}{c|}{0.882}          & 10.8          \\ \cline{5-12} 
                            &                               & \checkmark & \checkmark                  & \multicolumn{1}{c|}{3.17}          & \multicolumn{1}{c|}{4.35}          & \multicolumn{1}{c|}{0.954}          & 18.3          & \multicolumn{1}{c|}{2.00}          & \multicolumn{1}{c|}{2.50}          & \multicolumn{1}{c|}{0.892}          & 10.9          \\ \hline
\multirow{9}{*}{Generation} & \multirow{3}{*}{Demucs}       & &                   & \multicolumn{1}{c|}{2.84}          & \multicolumn{1}{c|}{3.91}          & \multicolumn{1}{c|}{0.944}          & 17.7          & \multicolumn{1}{c|}{1.65}          & \multicolumn{1}{c|}{2.11}          & \multicolumn{1}{c|}{0.870}          & 10.4          \\ \cline{5-12} 
                            &                               & \checkmark &                   & \multicolumn{1}{c|}{2.85}          & \multicolumn{1}{c|}{3.97}          & \multicolumn{1}{c|}{0.946}          & 17.5          & \multicolumn{1}{c|}{2.52}          & \multicolumn{1}{c|}{3.66}          & \multicolumn{1}{c|}{0.926}          & 14.5          \\ \cline{5-12} 
                            &                               & \checkmark & \checkmark                  & \multicolumn{1}{c|}{2.97}          & \multicolumn{1}{c|}{3.94}          & \multicolumn{1}{c|}{0.952}          & 16.5          & \multicolumn{1}{c|}{2.59}          & \multicolumn{1}{c|}{3.51}          & \multicolumn{1}{c|}{0.930}          & 13.3          \\ \cline{2-12} 
                            & \multirow{3}{*}{SE-Conformer} & &                   & \multicolumn{1}{c|}{2.80}          & \multicolumn{1}{c|}{4.00}          & \multicolumn{1}{c|}{0.944}          & \textbf{18.2} & \multicolumn{1}{c|}{1.64}          & \multicolumn{1}{c|}{2.22}          & \multicolumn{1}{c|}{0.868}          & 10.7          \\ \cline{5-12} 
                            &                               & \checkmark &                   & \multicolumn{1}{c|}{2.88}          & \multicolumn{1}{c|}{3.86}          & \multicolumn{1}{c|}{0.944}          & 16.8          & \multicolumn{1}{c|}{2.56}          & \multicolumn{1}{c|}{3.66}          & \multicolumn{1}{c|}{0.925}          & 13.9          \\ \cline{5-12} 
                            &                               & \checkmark &\checkmark              & \multicolumn{1}{c|}{3.08}          & \multicolumn{1}{c|}{3.99}          & \multicolumn{1}{c|}{0.952}          & 18.0          & \multicolumn{1}{c|}{\textbf{2.84}} & \multicolumn{1}{c|}{\textbf{3.86}} & \multicolumn{1}{c|}{\textbf{0.940}} & \textbf{15.5} \\ \cline{2-12} 
                            & \multirow{3}{*}{ConvTasNet}   & &        & \multicolumn{1}{c|}{2.88}          & \multicolumn{1}{c|}{3.91}          & \multicolumn{1}{c|}{0.947}          & 16.7          & \multicolumn{1}{c|}{1.74}          & \multicolumn{1}{c|}{2.26}          & \multicolumn{1}{c|}{0.876}          & 10.6          \\ \cline{5-12} 
                            &                               & \checkmark&                   & \multicolumn{1}{c|}{2.89}          & \multicolumn{1}{c|}{3.92}          & \multicolumn{1}{c|}{0.948}          & 13.9          & \multicolumn{1}{c|}{2.60}          & \multicolumn{1}{c|}{3.60}          & \multicolumn{1}{c|}{0.930}          & 12.9          \\ \cline{5-12} 
                            &                               & \checkmark & \checkmark               & \multicolumn{1}{c|}{\textbf{3.12}} & \multicolumn{1}{c|}{\textbf{4.12}} & \multicolumn{1}{c|}{\textbf{0.954}} & 12.8          & \multicolumn{1}{c|}{2.79}          & \multicolumn{1}{c|}{3.87}          & \multicolumn{1}{c|}{0.936}          & 12.0          \\ \hline
\end{tabular}
\caption{Speech restoration results on VCTK-DEMAND with and without degradation factors (noise, clipping, LPF, and silence gaps). Various network structures are compared according to the additional augmentation and the use of SSL representation.}
\label{t1:overall}
\end{table*}



\begin{table}[]
\fontsize{9pt}{12pt}
\selectfont
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Model}                                                                & \textbf{\begin{tabular}[c]{@{}c@{}}Cond. \\      method\end{tabular}} & \textbf{PESQ} & \textbf{NISQA} & \textbf{STOI}  \\ \hline
\multirow{3}{*}{SE-Conformer} & concat                                                                    & 2.84          & 3.86           & 0.940               \\ \cline{2-5} 
                                                                              & FiLM                                                                      & 2.84          & 3.81           & 0.938                   \\ \cline{2-5} 
                                                                              & sum                                                                       & 2.84          & 3.87           &    0.939                  \\ \hline
\multirow{3}{*}{ConvTasNet}                                                          & concat                                                                    & 2.79          & 3.87           & 0.936                 \\ \cline{2-5} 
                                                                              & FiLM                                                                      & 2.80          & 3.66           & 0.934                     \\ \cline{2-5} 
                                                                              & sum                                                                       & 2.75          & 3.84           &    0.935                      \\ \hline
\end{tabular}
\caption{Performance comparison by the different conditioning methods applied on SSL embedding to SE-Conformer network.}
\label{t2:condition}
\end{table}

